Recommended conventions for reporting results from direct dark matter searches

The field of dark matter detection is a highly visible and highly competitive one. In this paper, we propose recommendations for presenting dark matter direct detection results particularly suited for weak-scale dark matter searches, although we believe the spirit of the recommendations can apply more broadly to searches for other dark matter candidates, such as very light dark matter or axions. To translate experimental data into a final published result, direct detection collaborations must make a series of choices in their analysis, ranging from how to model astrophysical parameters to how to make statistical inferences based on observed data. While many collaborations follow a standard set of recommendations in some areas, for example the expected flux of dark matter particles (to a large degree based on a paper from Lewin and Smith in 1995), in other areas, particularly in statistical inference, they have taken different approaches, often from result to result by the same collaboration. We set out a number of recommendations on how to apply the now commonly used Profile Likelihood Ratio method to direct detection data. In addition, updated recommendations for the Standard Halo Model astrophysical parameters and relevant neutrino fluxes are provided. The authors of this note include members of the DAMIC, DarkSide, DARWIN, DEAP, LZ, NEWS-G, PandaX, PICO, SBC, SENSEI, SuperCDMS, and XENON collaborations, and these collaborations provided input to the recommendations laid out here. Wide-spread adoption of these recommendations will make it easier to compare and combine future dark matter results.

==> LZPaperSupport/LZsym.tex <==
%%%%%   Symbols for use in LZ
%%%%%
%%%%%   Revised from BaBar/SuperB/accelerator to LZ  08/17/2015  H. Nelson
%%%%%

\RequirePackage{xspace}

\RequirePackage{hyperref}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   KINEMATICS    %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\ptot       {\mbox{$p$}\xspace}
%\def\pxy        {\mbox{$p_{\mathrm{t}}$}
\def\pxy        {\mbox{$p_T$}\xspace}
%\def\pt         {\mbox{$p_{\mathrm{t}}$}\xspace}
\def\pt         {\mbox{$p_T$}\xspace}
\def\mes        {\mbox{$m_{\mathrm{ES}}$}\xspace}
\def\mec        {\mbox{$m_{\mathrm{EC}}$}\xspace}
\def\DeltaE     {\mbox{$\Delta E$}\xspace}

\def\pbcm {\ensuremath{p^*_{\Bz}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   GEOMETRY    %%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\mphi       {\mbox{$\phi$}\xspace}
\def\mtheta     {\mbox{$\theta$}\xspace}
\def\ctheta     {\mbox{$\cos\theta$}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% ENERGY AND MOMENTUM %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\newcommand{\keVee}{\si{\keV\ee}}
%\newcommand{\keVnr}{\si{\keV\nr}}
%\newcommand{\keVvis}{\si{\keV\vis}}
\DeclareRobustCommand{\Pga}{\HepParticle{\alpha}{}{}\xspace} % alpha
\DeclareRobustCommand{\Pgb}{\HepParticle{\beta}{}{}\xspace} % beta
\DeclareRobustCommand{\Pgd}{\HepParticle{\delta}{}{}\xspace} % delta
\DeclareRobustCommand{\Pgbm}{\HepParticle{\beta}{}{-}\xspace} % negative beta
\DeclareRobustCommand{\Pgbp}{\HepParticle{\beta}{}{+}\xspace} % positive beta
\DeclareRobustCommand{\Pd}{\HepParticle{d}{}{}\xspace} % deuteron
\DeclareRobustCommand{\Pad}{\HepAntiParticle{d}{}{}\xspace} % anti-deuteron
\DeclareRobustCommand{\Pt}{\HepParticle{t}{}{}\xspace} % triton
\DeclareRobustCommand{\Pad}{\HepAntiParticle{t}{}{}\xspace} % anti-triton
%\newcommand{\perkkd}{\si{\per\keV\per\kg\per\day}} % /keV/kg/day
%\newcommand{\perkgd}{\si{\per\keV\per\day}} % /kg/day
%\newcommand{\perktd}{\si{\per\keV\per\tonne\per\day}} % /keV/tonne/day
%\newcommand{\pertd}{\si{\per\tonne\per\day}} % /tonne/day
%\newcommand{\perkty}{\si{\per\keV\per\tonne\per\year}} % /keV/tonne/year
%\newcommand{\perty}{\si{\per\tonne\per\year}} % /tonne/year

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% DISTANCE AND AREA %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\syin {\ensuremath{^{\prime\prime}}\xspace}
\def\inch   {\ensuremath{\,\mathrfm{in}}\xspace} % \in is taken
\def\ft   {\ensuremath{\,\mathrfm{ft}}\xspace}
\def\km   {\ensuremath{{\,\mathrm{km}}}\xspace}
\def\m    {\ensuremath{{\,\mathrm{m}}}\xspace}
\def\msquare {\ensuremath{{\,\mathrm{m}}^2}\xspace}
\def\cm   {\ensuremath{{\,\mathrm{cm}}}\xspace}
\def\cma  {\ensuremath{{\,\mathrm{cm}}^2}\xspace}
\def\cubicm   {\ensuremath{{\,\mathrm{m}}^3}\xspace}
\def\mm   {\ensuremath{{\,\mathrm{mm}}}\xspace}
\def\mma  {\ensuremath{{\,\mathrm{mm}}^2}\xspace}
\def\mum  {\ensuremath{{\,\mu\mathrm{m}}}\xspace}%% mu meter
\def\muma {\ensuremath{{\,\mu\mathrm{m}}^2}\xspace}
\def\nm   {\ensuremath{{\,\mathrm{nm}}}\xspace}
\def\fm   {\ensuremath{{\,\mathrm{fm}}}\xspace}
\def\nm   {\ensuremath{{\,\mathrm{nm}}}\xspace}   %% nanometer
%
% integrated cross section, exposure
\def\barn{\ensuremath{{\,\mathrm{b}}}\xspace}
\def\barnhyph{\ensuremath{{\mathrm{-b}}}\xspace}
\def\mbarn{\ensuremath{{\,\mathrm{mb}}}\xspace}
\def\mbarnhyph{\ensuremath{{\rm -mb}}\xspace}
\def\nb{\ensuremath{{\,\mathrm{nb}}}\xspace}
\def\invnb {\ensuremath{\mbox{\,nb}^{-1}}\xspace}
\def\pb {\ensuremath{{\,\mathrm{pb}}}\xspace}
\def\invpb {\ensuremath{\mbox{\,pb}^{-1}}\xspace}
\def\fb   {\ensuremath{\mbox{\,fb}}\xspace}
\def\invfb   {\ensuremath{\mbox{\,fb}^{-1}}\xspace}
\def\ab   {\ensuremath{\mbox{\,ab}}\xspace}
\def\invab   {\ensuremath{\mbox{\,ab}^{-1}}\xspace}
\def\designlumi {\ensuremath{10^{36}\cms}\xspace}
\def\lumi {\cms\xspace}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% TIME AND MASS  %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\mus  {\ensuremath{\,\mus}\xspace}
\def\ns   {\ensuremath{\,\mathrm{ns}}\xspace}
\def\ps   {\ensuremath{\,\mathrm{ps}}\xspace}
\def\fs   {\ensuremath{\,\mathrm{fs}}\xspace}

%Mass
\def\gm   {\ensuremath{\,\mathrm{g}}\xspace}
\def\kg   {\ensuremath{\,\mathrfm{kg}}\xspace}
\def\ton  {\ensuremath{{\,\mathrm{t}}}\xspace}

\def\gmps {\ensuremath{\,\mathrm{g/s}}\xspace} 


%%\def\s{\ensuremath{\rm {\,s}}} %% second - this displays nothing  - why?
\def\sec{\ensuremath{{\,s}}\xspace}       %% second - this works - jw 4/19
\def\ms         {\ensuremath{{\,\mathrm{ms}}}\xspace}     %% millisecond
\def\mus        {\ensuremath{\,\mu\mathrm{s}}\xspace}    %% microsecond
\def\ns         {\ensuremath{{\,\mathrm{ns}}}\xspace}      %% nanosecond
\def\ps         {\ensuremath{{\,\mathrm{ps}}}\xspace}  %% picosecond


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%   MISCELLANEOUS %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\eg{\ensuremath\mathrm{e.g.}}
\def\ie{\ensuremath\mathrm{i.e.}}

\def\Xrad {\ensuremath{X_0}\xspace}
\def\NIL{\ensuremath{\lambda_{int}}\xspace}
\let\dgr\degrees

\def\pct {\ensuremath{{\,\mathrm{\%}}}\xspace}

\def\cms         {\ensuremath{{\,\mathrm{cm}}^{-2} {s}^{-1}}\xspace}

\def\muF  {\ensuremath{\,\mu\mathrm{F}}\xspace}
\def\muH  {\ensuremath{\,\mu\mathrm{H}}\xspace}
\def\nF   {\ensuremath{\,\mathrm{nF}}\xspace}
\def\nH   {\ensuremath{\,\mathrm{nH}}\xspace}
\def\mic  {\ensuremath{\,\mu\mathrm{C}}\xspace}
\def\krad {\ensuremath{\,\mathrm{krad}}\xspace}
\def\cmc  {\ensuremath{{\,\mathrm{cm}}^3}\xspace}
\def\yr   {\ensuremath{\,\mathrm{yr}}\xspace}
\def\hr   {\ensuremath{\,\mathrm{hr}}\xspace}
\def\degc {\ensuremath{^\circ}{\mathrm{C}}\xspace}
\def\degk {\ensuremath {\,\mathrm{K}}\xspace}
\def\degrees{\ensuremath{^{\circ}}\xspace}
\def\mrad{\ensuremath{\,\mathrm{mrad}}\xspace}               %% milliradian
\def\rad{\ensuremath{\,\mathrm{rad}}\xspace}
\def\mradhyph{\ensuremath{\mathrm{-mr}}\xspace}
%
\def\sx    {\ensuremath{\sigma_x}\xspace}
\def\sy    {\ensuremath{\sigma_y}\xspace}
\def\sz    {\ensuremath{\sigma_z}\xspace}
\def\thlf  {\ensuremath{\mathrm{T}_{1/2}}\xspace}

%\renewcommand{\bar}[1]{\overline{#1}}

% Some more (from Helen)
%\def\O{{\ensuremath{\cal O}}}  !!! This is a predefined LaTeX symbol !!!
\def\order{{\ensuremath{\cal O}}\xspace}
\def\L{{\ensuremath{\cal L}}\xspace}
\def\calL{{\ensuremath{\cal L}}\xspace}
%\def\S{{\ensuremath{\cal S}}}  !!! This is a predefined LaTeX symbol !!!
\def\calS{{\ensuremath{\cal S}}\xspace}
\def\calA{{\ensuremath{\cal A}}\xspace}
\def\calD{{\ensuremath{\cal D}}\xspace}
\def\calR{{\ensuremath{\cal R}}\xspace}

%% Arrows:
\def\ra                 {\ensuremath{\rightarrow}\xspace}
\def\to                 {\ensuremath{\rightarrow}\xspace}


\newcommand{\stat}{\ensuremath{\mathrm{(stat)}}\xspace}
\newcommand{\syst}{\ensuremath{\mathrm{(syst)}}\xspace}


\def\sx    {\ensuremath{\sigma_x}\xspace}
\def\sy    {\ensuremath{\sigma_y}\xspace}
\def\sz    {\ensuremath{\sigma_z}\xspace}


\newcommand{\inverse}{\ensuremath{^{-1}}\xspace}
\newcommand{\dedx}{\ensuremath{\mathrm{d}\hspace{-0.1em}E/\mathrm{d}x}\xspace}
\newcommand{\chisq}{\ensuremath{\chi^2}\xspace}
\newcommand{\delm}{\ensuremath{m_{\dstr}-m_{\dz}}\xspace}
\newcommand{\lum} {\ensuremath{\mathcal{L}}\xspace}

\def\gsim{{~\raise.15em\hbox{$>$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}
\def\lsim{{~\raise.15em\hbox{$<$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}

\def\qsq                {\ensuremath{q^2}\xspace}


% Data processing

\def\bit	{\ensuremath{{\,\text{bit}}}\xspace}
\def\kbit	{\ensuremath{{\,\text{kbit}}}\xspace}
\def\kbitps	{\ensuremath{{\,\text{kbit/s}}}\xspace}
\def\kbitsps	{\kbitps} % no more plural of units - deprecated
\def\kbps	{\kbitps} % for compatibility - deprecated
\def\kbsps	{\kbitsps} % for compatibility - deprecated

\def\kbyte      {\ensuremath{{\,\text{kByte}}}\xspace}
\def\kbytes	{\kbyte}
\def\kbyteps    {\ensuremath{{\,\text{kByte/s}}}\xspace}
\def\kbytesps	{\kbyteps}


\def\mbyte	{\ensuremath{{\,\text{MByte}}}\xspace}
\def\mbytes	{\mbyte}
\def\mbyteps	{\ensuremath{{\,\text{MByte/s}}}\xspace}
\def\mbytesps	{\mbyteps}

\def\mbit	{\ensuremath{{\,\text{Mbit}}}\xspace}
\def\mbits	{\mbit}
\def\mbitps	{\ensuremath{{\,\text{Mbit/s}}}\xspace}
\def\mbitsps	{\mbitps}
\def\mbps	{\mbitps} % for compatibility - deprecated
\def\mbsps	{\mbitsps} % for compatibility - deprecated

\def\gbit	{\ensuremath{{\,\text{Gbit}}}\xspace}
\def\gbits	{\gbit}
\def\gbitps	{\ensuremath{{\,\text{Gbit/s}}}\xspace}
\def\gbitsps	{\gbitps}
\def\gbps	{\gbitps} % for compatibility - deprecated
\def\gbsps	{\gbitsps} % for compatibility - deprecated


\def\gbyte	{\ensuremath{{\,\text{GByte}}}\xspace}
\def\gbytes	{\gbyte}
\def\gbyteps	{\ensuremath{{\,\text{GByte/s}}}\xspace}
\def\gbytesps	{\gbyteps}

\def\tbyte	{\ensuremath{{\,\text{TByte}}}\xspace}
\def\tbytes	{\tbyte}
\def\tbyteps	{\ensuremath{{\,\text{TByte/s}}}\xspace}
\def\tbytesps	{\tbyteps}
\def\tbyteph	{\ensuremath{{\,\text{TByte/h}}}\xspace}
\def\tbytesph   {\tbyteph}
\def\tbytepd	{\ensuremath{{\,\text{TByte/day}}}\xspace}
\def\tbytespd   {\tbytepd}

\def\pbyte	{\ensuremath{{\,\text{PByte}}}\xspace}
\def\pbytepy    {\ensuremath{{\,\text{PByte/yr}}}\xspace}

\def\tbpy       {\ensuremath{{\,\text{TByte/yr}}}\xspace}

\def\khs        {\ensuremath{{\,\text{kHS06}}}\xspace}
\def\mhs	{\ensuremath{{\,\text{MHS06}}}\xspace}

\def\tbpab	{\ensuremath{\tbyte/\invab}}
\def\khspab	{\ensuremath{\khs/\invab}}



\newcommand{\as}{\ensuremath{\alpha_{\scriptscriptstyle S}}\xspace}
\newcommand{\MSb}{\ensuremath{\overline{\mathrm{MS}}}\xspace}
\newcommand{\LMSb}{%
  \ensuremath{\Lambda_{\overline{\scriptscriptstyle\mathrm{MS}}}}\xspace
}

% Electroweak parameters

\newcommand{\tw}{\ensuremath{\theta_{\scriptscriptstyle W}}\xspace}
\newcommand{\twb}{\ensuremath{\overline{\theta}_{\scriptscriptstyle W}}\xspace}
\newcommand{\Afb}[1]{{\ensuremath{A_{\scriptscriptstyle FB}^{#1}}}\xspace}
\newcommand{\gv}[1]{{\ensuremath{g_{\scriptscriptstyle V}^{#1}}}\xspace}
\newcommand{\ga}[1]{{\ensuremath{g_{\scriptscriptstyle A}^{#1}}}\xspace}
\newcommand{\gvb}[1]{{\ensuremath{\overline{g}_{\scriptscriptstyle V}^{#1}}}\xspace}
\newcommand{\gab}[1]{{\ensuremath{\overline{g}_{\scriptscriptstyle A}^{#1}}}\xspace}

%\newcommand{\eqref}[1]{Eq.~(\ref{eq:#1})}
\newcommand{\secref}[1]{Section~\ref{sec:#1}}
\newcommand{\subsecref}[1]{Section~\ref{subsec:#1}}
\newcommand{\figref}[1]{Figure~\ref{fig:#1}}
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}

%
% Dark Matter
%
\newcommand{\vesc}{\ensuremath{v_{\text{esc}}}\xspace}
\newcommand{\MWIMP}{\ensuremath{M_{\text{WIMP}}}\xspace}
\newcommand{\Emin}{\ensuremath{E_{\text{min}}}\xspace}
\newcommand{\QBB}{\ensuremath{Q_{\!\Pgb\kern-0.1em\Pgb}}\xspace}

%
% Radioactive Isotopes
%
\newcommand{\IXenat}{\HepIsotope{Xe}{}{nat}\xspace}
\newcommand{\IXemes}{\HepIsotope{Xe}{}{m}\xspace}
\newcommand{\IXeotf}{\HepIsotope{Xe}{}{124}\xspace}
\newcommand{\IXeotF}{\HepIsotope{Xe}{}{125}\xspace}
\newcommand{\IXeots}{\HepIsotope{Xe}{}{126}\xspace}
\newcommand{\IXeotS}{\HepIsotope{Xe}{}{127}\xspace}
\newcommand{\IXeote}{\HepIsotope{Xe}{}{128}\xspace}
\newcommand{\IXeotn}{\HepIsotope{Xe}{}{129}\xspace}
\newcommand{\IXeotnm}{\HepIsotope{Xe}{}{129m}\xspace}
\newcommand{\IXeoTz}{\HepIsotope{Xe}{}{130}\xspace}
\newcommand{\IXeoTo}{\HepIsotope{Xe}{}{131}\xspace}
\newcommand{\IXeoTom}{\HepIsotope{Xe}{}{131m}\xspace}
\newcommand{\IXeoTt}{\HepIsotope{Xe}{}{132}\xspace}
\newcommand{\IXeoTT}{\HepIsotope{Xe}{}{133}\xspace}
\newcommand{\IXeoTf}{\HepIsotope{Xe}{}{134}\xspace}
\newcommand{\IXeoTF}{\HepIsotope{Xe}{}{135}\xspace}
\newcommand{\IXeoTs}{\HepIsotope{Xe}{}{136}\xspace}
\newcommand{\IKrnat}{\HepIsotope{Kr}{}{nat}\xspace}
\newcommand{\IKreF}{\HepIsotope{Kr}{}{85}\xspace}
\newcommand{\IKreTm}{\HepIsotope{Kr}{}{83m}\xspace}
\newcommand{\IKreT}{\HepIsotope{Kr}{}{83}\xspace}
\newcommand{\IRbeT}{\HepIsotope{Rb}{}{83}\xspace}
\newcommand{\IRntoe}{\HepIsotope{Rn}{}{218}\xspace}
\newcommand{\IRnton}{\HepIsotope{Rn}{}{219}\xspace}
\newcommand{\IRnttz}{\HepIsotope{Rn}{}{220}\xspace}
\newcommand{\IRnttt}{\HepIsotope{Rn}{}{222}\xspace}
\newcommand{\IHo}{\HepIsotope{H}{}{1}\xspace}
\newcommand{\IHt}{\HepIsotope{H}{}{2}\xspace}
\newcommand{\IHT}{\HepIsotope{H}{}{3}\xspace}
\newcommand{\IHeT}{\HepIsotope{He}{}{3}\xspace}
\newcommand{\IArTS}{\HepIsotope{Ar}{}{37}\xspace}
\newcommand{\IArTn}{\HepIsotope{Ar}{}{39}\xspace}
\newcommand{\IArnat}{\HepIsotope{Ar}{}{nat}\xspace}
\newcommand{\IUtTf}{\HepIsotope{U}{}{234}\xspace}
\newcommand{\IUtTF}{\HepIsotope{U}{}{235}\xspace}
\newcommand{\IUtTe}{\HepIsotope{U}{}{238}\xspace}
\newcommand{\IUtTeE}{\HepIsotope{U}{}{238}$_{\mathrm{e}}$\xspace}
\newcommand{\IUtTeL}{\HepIsotope{U}{}{238}$_{\mathrm{l}}$\xspace}
\newcommand{\IUnat}{\HepIsotope{U}{}{nat}\xspace}
\newcommand{\IPatTo}{\HepIsotope{Pa}{}{231}\xspace}
\newcommand{\IPatTT}{\HepIsotope{Pa}{}{233}\xspace}
\newcommand{\IPatTf}{\HepIsotope{Pa}{}{234}\xspace}
\newcommand{\IPatTfm}{\HepIsotope{Pa}{}{234m}\xspace}
\newcommand{\IThttS}{\HepIsotope{Th}{}{227}\xspace}
\newcommand{\IThtte}{\HepIsotope{Th}{}{228}\xspace}
\newcommand{\IThtTz}{\HepIsotope{Th}{}{230}\xspace}
\newcommand{\IThtTo}{\HepIsotope{Th}{}{231}\xspace}
\newcommand{\IThtTt}{\HepIsotope{Th}{}{232}\xspace}
\newcommand{\IThtTtE}{\HepIsotope{Th}{}{232}$_{\mathrm{e}}$\xspace}
\newcommand{\IThtTtL}{\HepIsotope{Th}{}{232}$_{\mathrm{l}}$\xspace}
\newcommand{\IThtTf}{\HepIsotope{Th}{}{234}\xspace}
\newcommand{\IActtS}{\HepIsotope{Ac}{}{227}\xspace}
\newcommand{\IActte}{\HepIsotope{Ac}{}{228}\xspace}
\newcommand{\IRattT}{\HepIsotope{Ra}{}{223}\xspace}
\newcommand{\IRattf}{\HepIsotope{Ra}{}{224}\xspace}
\newcommand{\IRatts}{\HepIsotope{Ra}{}{226}\xspace}
\newcommand{\IRattS}{\HepIsotope{Ra}{}{227}\xspace}
\newcommand{\IRatte}{\HepIsotope{Ra}{}{228}\xspace}
\newcommand{\IFrttT}{\HepIsotope{Fr}{}{223}\xspace}
\newcommand{\IFrttf}{\HepIsotope{Fr}{}{224}\xspace}
\newcommand{\IAttoF}{\HepIsotope{At}{}{215}\xspace}
\newcommand{\IAttoe}{\HepIsotope{At}{}{218}\xspace}
\newcommand{\IAtton}{\HepIsotope{At}{}{219}\xspace}
\newcommand{\IPotoz}{\HepIsotope{Po}{}{210}\xspace}
\newcommand{\IPotoo}{\HepIsotope{Po}{}{211}\xspace}
\newcommand{\IPotot}{\HepIsotope{Po}{}{212}\xspace}
\newcommand{\IPotof}{\HepIsotope{Po}{}{214}\xspace}
\newcommand{\IPotoF}{\HepIsotope{Po}{}{215}\xspace}
\newcommand{\IPotos}{\HepIsotope{Po}{}{216}\xspace}
\newcommand{\IPotoe}{\HepIsotope{Po}{}{218}\xspace}
\newcommand{\IBitzF}{\HepIsotope{Bi}{}{205}\xspace}
\newcommand{\IBitzs}{\HepIsotope{Bi}{}{206}\xspace}
\newcommand{\IBitoz}{\HepIsotope{Bi}{}{210}\xspace}
\newcommand{\IBitoo}{\HepIsotope{Bi}{}{211}\xspace}
\newcommand{\IBitot}{\HepIsotope{Bi}{}{212}\xspace}
\newcommand{\IBitof}{\HepIsotope{Bi}{}{214}\xspace}
\newcommand{\IBitoF}{\HepIsotope{Bi}{}{215}\xspace}
\newcommand{\IPbtzs}{\HepIsotope{Pb}{}{206}\xspace}
\newcommand{\IPbtzS}{\HepIsotope{Pb}{}{207}\xspace}
\newcommand{\IPbtze}{\HepIsotope{Pb}{}{208}\xspace}
\newcommand{\IPbtoz}{\HepIsotope{Pb}{}{210}\xspace}
\newcommand{\IPbtot}{\HepIsotope{Pb}{}{212}\xspace}
\newcommand{\IPbtof}{\HepIsotope{Pb}{}{214}\xspace}
\newcommand{\ITltzs}{\HepIsotope{Tl}{}{206}\xspace}
\newcommand{\ITltzS}{\HepIsotope{Tl}{}{207}\xspace}
\newcommand{\ITltze}{\HepIsotope{Tl}{}{208}\xspace}
\newcommand{\ITltoz}{\HepIsotope{Tl}{}{210}\xspace}
\newcommand{\IHgtos}{\HepIsotope{Hg}{}{206}\xspace}
\newcommand{\IKfz}{\HepIsotope{K}{}{40}\xspace}
\newcommand{\IKnat}{\HepIsotope{K}{}{nat}\xspace}
\newcommand{\IScfs}{\HepIsotope{Sc}{}{46}\xspace}
\newcommand{\ICoFS}{\HepIsotope{Co}{}{57}\xspace}
\newcommand{\IKft}{\HepIsotope{K}{}{42}\xspace}
\newcommand{\IScffm}{\HepIsotope{Sc}{}{44,44m}\xspace}
\newcommand{\IScfS}{\HepIsotope{Sc}{}{47}\xspace}
\newcommand{\IScfe}{\HepIsotope{Sc}{}{48}\xspace}
\newcommand{\ICsoTS}{\HepIsotope{Cs}{}{137}\xspace}
\newcommand{\ICftFt}{\HepIsotope{Cf}{}{252}\xspace}
\newcommand{\ICosz}{\HepIsotope{Co}{}{60}\xspace}
\newcommand{\ICrFo}{\HepIsotope{Cr}{}{51}\xspace}
\newcommand{\IAmtfo}{\HepIsotope{Am}{}{241}\xspace}
\newcommand{\IYee}{\HepIsotope{Y}{}{88}\xspace}
\newcommand{\ICsoTs}{\HepIsotope{Cs}{}{136}\xspace}
\newcommand{\INatt}{\HepIsotope{Na}{}{22}\xspace}
\newcommand{\IBe}{\HepIsotope{B}{}{8}\xspace}
\newcommand{\IBeS}{\HepIsotope{Be}{}{7}\xspace}
\newcommand{\IBen}{\HepIsotope{Be}{}{9}\xspace}
\newcommand{\INoT}{\HepIsotope{N}{}{13}\xspace}
\newcommand{\INof}{\HepIsotope{N}{}{14}\xspace}
\newcommand{\IOoF}{\HepIsotope{O}{}{15}\xspace}
\newcommand{\IFoS}{\HepIsotope{F}{}{17}\xspace}
\newcommand{\Ipp}{\HepIsotope{p}{}{}\HepIsotope{p}{}{}\xspace}
\newcommand{\Ihep}{\HepIsotope{h}{}{}\HepIsotope{e}{}{}\HepIsotope{p}{}{}\xspace}
\newcommand{\Dnuenue}{\hbox{\Pgn\kern-0.3em\Pe\kern-0.3em$\to$\kern-0.1em\Pgn\kern-0.3em\Pe}\xspace}
\newcommand{\ISmofS}{\HepIsotope{Sm}{}{147}\xspace}
\newcommand{\ISmoFz}{\HepIsotope{Sm}{}{150}\xspace}
\newcommand{\ISmoFT}{\HepIsotope{Sm}{}{153}\xspace}
\newcommand{\IEuoFt}{\HepIsotope{Eu}{}{152}\xspace}
\newcommand{\IGd}{\HepIsotope{Gd}{}{}\xspace}
\newcommand{\IGdnat}{\HepIsotope{Gd}{}{nat}\xspace}
\newcommand{\IGdoFt}{\HepIsotope{Gd}{}{152}\xspace}
\newcommand{\IGdoFT}{\HepIsotope{Gd}{}{153}\xspace}
\newcommand{\IGdoFf}{\HepIsotope{Gd}{}{154}\xspace}
\newcommand{\IGdoFF}{\HepIsotope{Gd}{}{155}\xspace}
\newcommand{\IGdoFs}{\HepIsotope{Gd}{}{156}\xspace}
\newcommand{\IGdoFS}{\HepIsotope{Gd}{}{157}\xspace}
\newcommand{\IGdoFe}{\HepIsotope{Gd}{}{158}\xspace}
\newcommand{\IGdosz}{\HepIsotope{Gd}{}{160}\xspace}
\newcommand{\ICot}{\HepIsotope{C}{}{12}\xspace}
\newcommand{\ICoT}{\HepIsotope{C}{}{13}\xspace}
\newcommand{\ICof}{\HepIsotope{C}{}{14}\xspace}
\newcommand{\ILaoTe}{\HepIsotope{La}{}{138}\xspace}
\newcommand{\INptTn}{\HepIsotope{Np}{}{239}\xspace}
\newcommand{\ICsoTf}{\HepIsotope{Cs}{}{134}\xspace}
\newcommand{\IIotF}{\HepIsotope{I}{}{125}\xspace}
\newcommand{\IIotS}{\HepIsotope{I}{}{127}\xspace}
\newcommand{\IIoTo}{\HepIsotope{I}{}{131}\xspace}
\newcommand{\ITeotom}{\HepIsotope{Te}{}{121m}\xspace}
\newcommand{\ITeotTm}{\HepIsotope{Te}{}{123m}\xspace}
%
%  Double Beta Decay
%
%\newcommand{\Pznbb}{\hbox{0\Pgn\kern-4pt\Pgb\kern-4pt\Pgb}}
\newcommand{\Dznbb}{\hbox{0\Pgn\kern-0.3em\Pgb\kern-0.35em\Pgb}\xspace}
\newcommand{\Dtnbb}{\hbox{2\Pgn\kern-0.3em\Pgb\kern-0.35em\Pgb}\xspace}

%
% Chemicals - intially single elements
%
\newcommand{\CNt}{\HepChemical{N}{2}{}\xspace}
\newcommand{\COt}{\HepChemical{O}{2}{}\xspace}
\newcommand{\COtM}{\HepChemical{O}{2}{-}\xspace}
\newcommand{\CHt}{\HepChemical{H}{2}{}\xspace}
\newcommand{\CHT}{\HepChemical{H}{3}{}\xspace}
\newcommand{\CHf}{\HepChemical{H}{4}{}\xspace}
\newcommand{\CHFi}{\HepChemical{H}{5}{}\xspace}
\newcommand{\CHs}{\HepChemical{H}{6}{}\xspace}
\newcommand{\CHoo}{\HepChemical{H}{11}{}}
\newcommand{\CHot}{\HepChemical{H}{12}{}\xspace}
\newcommand{\CHos}{\HepChemical{H}{16}{}\xspace}
\newcommand{\CHoS}{\HepChemical{H}{17}{}\xspace}
\newcommand{\CHtt}{\HepChemical{H}{22}{}\xspace}
\newcommand{\CHGdLS}{\HepChemical{H}{28.128}{}\xspace}
\newcommand{\CHLAB}{\HepChemical{H}{28.28}{}\xspace}
\newcommand{\CHtN}{\HepChemical{H}{2n}{}\xspace}
\newcommand{\CCs}{\HepChemical{C}{6}{}\xspace}
\newcommand{\CCn}{\HepChemical{C}{9}{}\xspace}
\newcommand{\CCoF}{\HepChemical{C}{15}{}\xspace}
\newcommand{\CCGdLS}{\HepChemical{C}{17.072}{}\xspace}
\newcommand{\CCLAB}{\HepChemical{C}{17.14}{}\xspace}
\newcommand{\CCtf}{\HepChemical{C}{24}{}\xspace}
\newcommand{\CCN}{\HepChemical{C}{n}{}\xspace}
\newcommand{\COGdLS}{\HepChemical{O}{0.0126}{}\xspace}
\newcommand{\CNGdLS}{\HepChemical{N}{0.0037}{}\xspace}
\newcommand{\CGdGdLS}{\HepChemical{Gd}{0.0015}{}\xspace}
\newcommand{\CClT}{\HepChemical{Cl}{3}{}\xspace}
\newcommand{\CCrt}{\HepChemical{Cr}{2}{}\xspace}
\newcommand{\COT}{\HepChemical{O}{3}{}\xspace}
\newcommand{\CAlt}{\HepChemical{Al}{2}{}\xspace}
%
% Chemicals - Compounds
%
\newcommand{\CCsHF}{\CCs\kern-0.2em\CHFi}
\newcommand{\CCnHot}{\CCn\kern-0.2em\CHot}
\newcommand{\CCH}{CH\xspace}
\newcommand{\CCNHtN}{\CCN\kern-0.2em\CHtN}
\newcommand{\CCHLAB}{\CCLAB\kern-0.2em\CHLAB}
\newcommand{\CHtO}{\CHt{O}\xspace}
\newcommand{\CGdClT}{Gd\CClT\xspace}
\newcommand{\CHF}{HF\xspace}
\newcommand{\CHCl}{HCl\xspace}
\newcommand{\CCrtOT}{\CCrt\kern-0.25em\COT}
\newcommand{\CHNOT}{HN\COT}
\newcommand{\CAltOT}{\CAlt\kern-0.25em\COT}
\newcommand{\CBaTiOT}{BaTi\kern0.05em\COT}
\newcommand{\CNaI}{NaI\xspace}
\newcommand{\CCHt}{\HepChemical{C}{}{}\CHt}
\newcommand{\CCHT}{\HepChemical{C}{}{}\CHT}
\newcommand{\CCHf}{\HepChemical{C}{}{}\CHf}
\newcommand{\CTMHA}{\CCn\kern-0.2em\CHoS\kern-0.2em\COt}
\newcommand{\CTMHAm}{\CCn\kern-0.2em\CHos\kern-0.2em\COt}
\newcommand{\CTMHAM}{\CCn\kern-0.2em\CHos\kern-0.2em\COtM}
\newcommand{\CPPO}{\CCoF\kern-0.2em\CHoo NO}
\newcommand{\CbisMSB}{\CCtf\kern-0.2em\CHtt}
\newcommand{\CGdLS}{\CCGdLS\kern-0.2em\CHGdLS\kern-0.2em\COGdLS\kern-0.2em\CNGdLS\kern-0.2em\CGdGdLS}
%
% Table-related
%
\colorlet{mrocol}{ProcessBlue!100!}
\colorlet{lrocol}{SkyBlue!50!}
\newcommand{\sfbL}{\sffamily\bfseries\Large}
\newcommand{\sfbl}{\sffamily\bfseries\large}
\newcommand{\sfs}{\sffamily\small}
\newcommand{\rmbL}{\rmfamily\bfseries\Large}
\newcommand{\rmbl}{\rmfamily\bfseries\large}
\newcommand{\rms}{\rmfamily\small}
\newcommand{\Tstrut}{\rule{0pt}{2.4ex}}
\newcommand{\Bstrut}{\rule{1ex}{0pt}}
\newcommand{\numlb}[1]{\num[color=Tan]{#1}}
\newcolumntype{L}[1]{>{\raggedright\arraybackslash}m{#1}}
\newcolumntype{C}[1]{>{\centering\arraybackslash}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\arraybackslash}m{#1}}

%%%%%%%%%%%%%%%%%%%% SOFTWARE PACKAGES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\aslund     {\mbox{\tt Aslund}\xspace}
\def\bbsim      {\mbox{\tt BBsim}\xspace}
\def\beast      {\mbox{\tt Beast}\xspace}
\def\beget      {\mbox{\tt Beget}\xspace}
\def\Bta        {\mbox{\tt Beta}\xspace}
\def\betakfit   {\mbox{\tt BetaKfit}\xspace}
\def\cornelius  {\mbox{\tt Cornelius}\xspace}
\def\evtgen     {\mbox{\tt EvtGen}\xspace}
\def\euclid     {\mbox{\tt Euclid}\xspace}
\def\fitver     {\mbox{\tt FitVer}\xspace}
\def\fluka      {\mbox{\tt Fluka}\xspace}
\def\fortran    {\mbox{\tt Fortran}\xspace}
\def\gcalor     {\mbox{\tt GCalor}\xspace}
\def\geant      {\mbox{\tt GEANT}\xspace}
%\def\geantFour  {\mbox{\tt GEANT4}\xspace}
\def\geantFour  {\mbox{\scshape Geant4}\xspace}
\def\gheisha    {\mbox{\tt Gheisha}\xspace}
\def\hemicosm   {\mbox{\tt HemiCosm}\xspace}
\def\hepevt     {\mbox{\tt{/HepEvt/}}\xspace}
\def\jetset74   {\mbox{\tt Jetset \hspace{-0.5em}7.\hspace{-0.2em}4}\xspace}
%\def\jetset     {\mbox{\tt Jetset \hspace{-0.5em}7.\hspace{-0.2em}4}}
\def\koralb     {\mbox{\tt KoralB}\xspace}
\def\minuit     {\mbox{\tt Minuit}\xspace}
\def\objegs     {\mbox{\tt Objegs}\xspace}
\def\paw        {\mbox{\tt Paw}\xspace}
\def\Root       {\mbox{\tt Root}\xspace}
\def\squaw      {\mbox{\tt Squaw}\xspace}
\def\stdhep     {\mbox{\tt StdHep}\xspace}
\def\trackerr   {\mbox{\tt TrackErr}\xspace}
\def\turtle     {\mbox{\tt Decay~Turtle}\xspace}
%
%  From Accelerator
%
\def\tenTo#1#2{\ensuremath{10^{#1#2} \cms}\xspace}
\newcommand{\EE}[1] {\ensuremath{\times 10^{#1}}\xspace}
\newcommand{\EEb}[1] {\ensuremath{\times \mathbf{10}^{\mathbf{#1}}}\xspace}
\newcommand{\PM}[2] {\ensuremath{^{+#1}_{-#2}}\xspace}

% Spin Polarization common symbols
\def\ze#1   {\ensuremath{\zeta_{#1}}\xspace}
\newcommand{\VE}[1]  {\ensuremath{\vec{\mathrm{#1}}}\xspace}

% Electrical units
\def\amp    {\ensuremath{{\rm \,\mathrm{A}}}\xspace}
\def\mA     {\ensuremath{{\rm \,\mathrm{mA}}}\xspace}
\def\muA     {\ensuremath{\mu\mathrm{A}}\xspace}
\def\kA	    {\ensuremath{{\,\mathrm{kA}}}\xspace}
\def\nC     {\ensuremath{{\,\mathrm{nC}}}\xspace}
\def\pC     {\ensuremath{{\,\mathrm{pC}}}\xspace}
\def\Ohm    {\ensuremath{{\,\Omega}}\xspace}
\def\mOhm   {\ensuremath{{\,\mathrm{m}\Omega}}\xspace}
\def\kOhm   {\ensuremath{{\,\mathrm{k}\Omega}}\xspace}
\def\MOhm   {\ensuremath{{\,\mathrm{M}\Omega}}\xspace}
\def\V     {\ensuremath{{\,\mathrm{V}}}\xspace}
\def\kV     {\ensuremath{{\,\mathrm{kV}}}\xspace}
\def\MV     {\ensuremath{{\,\mathrm{MV}}}\xspace}
\def\mV     {\ensuremath{{\,\mathrm{mV}}}\xspace}	
\def\Tesla  {\ensuremath{{\,\mathrm{T}}}\xspace}
\def\Gauss  {\ensuremath{{\,\mathrm{G}}}\xspace}
\def\kGauss  {\ensuremath{{\,\mathrm{kG}}}\xspace}
\def\dB     {\ensuremath{{\,\mathrm{dB}}}\xspace}
\def\Henry  {\ensuremath{{\,\mathrm{H}}}\xspace}

% SI energy unit
\def\J      {\ensuremath{{\,\mathrm{J}}}\xspace}
\def\kJ     {\ensuremath{{\,\mathrm{kJ}}}\xspace}
\def\MJ     {\ensuremath{{\,\mathrm{MJ}}}\xspace}

\def\Jpgm   {\ensuremath{{\,\mathrm{J/g}}}\xspace}

% Power
\def\Watt      {\ensuremath{{\,\mathrm{W}}}\xspace}
\def\MW     {\ensuremath{{\,\mathrm{MW}}}\xspace}
\def\kW     {\ensuremath{{\,\mathrm{kW}}}\xspace}


% Frequency
\def\Hz     {\ensuremath{{\rm \,Hz}}\xspace}
\def\MHz    {\ensuremath{{\rm \,MHz}}\xspace}
\def\GHz    {\ensuremath{{\rm \,GHz}}\xspace}
\def\kHz    {\ensuremath{{\rm \,kHz}}\xspace}

% Flux
\def\Hzpmma {\ensuremath{{\rm \,Hz/mm^2}}\xspace}
\def\kHzpmma {\ensuremath{{\rm \,kHz/mm^2}}\xspace}

\def\Hzpcma {\ensuremath{{\rm \,Hz/cm^2}}\xspace}
\def\kHzpcma {\ensuremath{{\rm \,kHz/cm^2}}\xspace}

% Neutron fluence, flux
\def\neqpcma {\ensuremath{{\,{\rm n}_{eq}/{\rm cm^2}}}\xspace}
\def\neqpcmaps  {\ensuremath{{\,{\rm n}_{eq}/{\rm cm^2/s}}}\xspace}
\def\neqpcmapyr  {\ensuremath{{\,{\rm n}_{eq}/{\rm cm^2/yr}}}\xspace}



% Time
\def\msec   {\ensuremath{{\rm \,ms}}\xspace}
\def\nsec   {\ensuremath{{\rm \,ns}}\xspace}

% Pressure
\def\Torr  {\ensuremath{{\rm \,Torr}}\xspace}
\def\nTorr  {\ensuremath{{\rm \,nTorr}}\xspace}
\def\Pa     {\ensuremath{{\rm \,Pa}}\xspace}
\def\MPa    {\ensuremath{{\rm \,MPa}}\xspace}

% Length
\def\picom  {\ensuremath{{\rm \,pm}}\xspace}
\def\km  {\ensuremath{{\rm \,km}}\xspace}

% Area
%(in babarsym) \def\mbarn  {\ensuremath{{\rm \,mbarn}}\xspace}

% Angle
\def\muRad  {\ensuremath{{\, \mu \rm rad}}\xspace}

% Force
\def\N     {\ensuremath{{\rm \,N}}\xspace}
\def\kN    {\ensuremath{{\rm \,kN}}\xspace} 
\def\kNpmm {\ensuremath{{\rm \,kN/mm}}\xspace}


\def\bets  {\ensuremath{{\beta^{\star}}}\xspace}
\def\betxs  {\ensuremath{{\beta_{x}^{\star}}}\xspace}
\def\betys  {\ensuremath{{\beta_{y}^{\star}}}\xspace}

\def\betx   {\ensuremath{{\beta_{x}}}\xspace}
\def\bety   {\ensuremath{{\beta_{y}}}\xspace}


\def\epsx   {\ensuremath{{\varepsilon_{x}}}\xspace}
\def\epsy   {\ensuremath{{\varepsilon_{y}}}\xspace}

\def\xix  {\ensuremath{{\xi_{x}}}\xspace}
\def\xiy  {\ensuremath{{\xi_{y}}}\xspace}

\def\thx  {\ensuremath{{\theta}}\xspace}
\def\piwi {\ensuremath{{\varphi}}\xspace}
\def\CW   {CW\xspace}
\def\br   {\ensuremath{B\rho}\xspace}
\def\thr  {\ensuremath{\theta_{r}}\xspace}

% Note: original symbol Bz conflicts with what is defined in babarsym
\def\Bzed   {\ensuremath{B_{z}}\xspace}

\def\Be   {Be\xspace}
\def\Cu   {Cu\xspace}
\def\Au   {Au\xspace}
\def\CO2  {$\mathrm{CO}_2$\xspace}


\newcommand{\TODO}[1] {{\color{red} \mbox{ #1}}\xspace}


% Note: for Debbie Ceder, 10/8/2015
%\newcommand{\gtwid}{\mathrel{\raise.3ex\hbox{$>$\kern-.75em\lower1ex\hbox{$\sim$}}}}
%\newcommand{\ltwid}{\mathrel{\raise.3ex\hbox{$<$\kern-.75em\lower1ex\hbox{$\sim$}}}}


==> LZPaperSupport/commands.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% SuperB Detector Technical Design Report
% User defined commands and symbols
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Define symbols
\input{LZsym}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Define command to begin new section/subsection/subsubsection, so that it's easy to change it
% Use:
% \tdrchap for the chapter/subsystem level
%  \tdrsec for the section level
%     \tdrsubsec
%        \tdrsubsubsec
%           \tdrparagraph
%
% Command to include chapters. Convention is that the main file name is the same as the chapter directory
% For example : SVT/SVT.tex
% This requires the 'import' package that takes care of handling the subdirectories
% \subimport* means include from subdir without looking in TEXINPUTS
% Used in conjuction of the \tdrchap command, it automatically defines a chapter
% label, in the form of chap:dirname, such as \label{chap:SVT} 
%
\newcommand{\ChapLabel}{chap:empty}
\newcommand{\BibLabel}{empty:bib}
\newcommand{\SecPre}{empty}
\newcommand{\FloatPre}{empty}
\newcommand{\tdrinclude}[1]
{
%\befchap
\renewcommand{\ChapLabel}{chap:#1} % define the label for the chapter
\renewcommand{\BibLabel}{#1S:bib} % define the label for the chapter
\renewcommand{\SecPre}{#1}
\renewcommand{\FloatPre}{#1}
\subincludefrom{#1/}{#1}
\wlog{In tdrinclude command}
\wlog{\ChapLabel}
%\aftchap
}

\newcommand{\tdrchap}[2][\ChapLabel]
{
   \ifx#1\ChapLabel
     \chapter{#2\ifKL\space\texttt{#1}\fi}
     \label{#1}
   \else
    \renewcommand{\ChapLabel}{chap:#1} % define the label for the chapter
    \renewcommand{\BibLabel}{#1S:bib} % define the label for the chapter
    \renewcommand{\SecPre}{#1}
    \renewcommand{\FloatPre}{#1}
    \chapter{#2\ifKL\space\texttt{\ChapLabel}\fi}
    \label{\ChapLabel}
   \fi
}

\newcommand{\tdrsec}[2][\Alph{section}]
{
   \section{#2\ifKL\space\texttt{\SecPre S:#1}\fi}
   \label{\SecPre S:#1}
}

\newcommand{\tdrsubsec}[2][\Alph{section}\alph{subsection}]
{
   \subsection{#2\ifKL\space\texttt{\SecPre Ss:#1}\fi}
   \label{\SecPre Ss:#1}
}

\newcommand{\tdrsubsubsec}[2][\Alph{section}\alph{subsection}\Roman{subsubsection}]
{
   \subsubsection{#2\ifKL\space\texttt{\SecPre Sss:#1}\fi}
   \label{\SecPre Sss:#1}   
}

\newcommand{\tdrparagraph}[2][\Alph{section}\alph{subsection}\Roman{subsubsection}\roman{paragraph}]
{
   \paragraph{#2\ifKL\space\texttt{\SecPre Sssp:#1}\fi}
   \label{\SecPre Sssp:#1}
}

\renewcommand{\bibsection}{\tdrsec[bib]{Bibliography}}

\newcommand{\tdrtcaption}[3][\arabic{section}.\arabic{subsection}.\arabic{table}]
{
   \caption[#2\ifKL\space\texttt{\FloatPre t:#1}\fi]{#3\ifKL\space\texttt{\FloatPre t:#1}\fi}
   \label{\FloatPre t:#1}
}

\newcommand{\tdrfcaption}[3][\arabic{section}.\arabic{subsection}.\arabic{figure}]
{
   \caption[#2\ifKL\space\texttt{\FloatPre f:#1}\fi]{#3\ifKL\space\texttt{\FloatPre f:#1}\fi}
   \label{\FloatPre f:#1}
}

%\iftrue
%\titleformat{\section}%
%  {\raggedsection\normalfont\sectfont\Large\bfseries}%{\thesection}%
%  {0.4em}%
%  {\phantomsection}%
%  [\vspace{0.5ex}\centerline{\rule[0.15in]{0.9\columnwidth}{2pt}}\vspace*{-1.5ex}]
%\fi

%%%
% Define the detpth for numbering sections and including them in TOC
%
\setcounter{secnumdepth}{3}
\setcounter{tocdepth}{3}

%
% commands handling new page at the end of chapters
%
\newcommand{\befchap}{\relax}
\newcommand{\aftchap}{\relax}
%

\long\def\ignore#1{\relax}
\let\BaBar=\babar

%%--- define \url font to be small normal font
%\makeatletter
%\def\url@tdrstyle{%
%  \@ifundefined{selectfont}{\def\UrlFont{\normalfont}}{\def\UrlFont{\normalfont\smaller}}}
%\makeatother
%\urlstyle{tdr}
%%\urlstyle{same}

%%--- put bibliography in a section for scrbook
\makeatletter
\renewcommand*\bib@heading{%
  \section{\bibname}
  \@mkboth{\bibname}{\bibname}
}
\makeatother

%%
%% floats
%%

\renewcommand{\topfraction}{.85} % max fraction of floats at top
\renewcommand{\bottomfraction}{.70} % max fraction of floats at bottom
\renewcommand{\textfraction}{.15}
\renewcommand{\floatpagefraction}{.66} % float-only pages
\renewcommand{\dbltopfraction}{.66}
\renewcommand{\dblfloatpagefraction}{.66} % float-only pages

%%--- max number of floats in text pages
\setcounter{topnumber}{9}
\setcounter{bottomnumber}{9}
\setcounter{totalnumber}{20}
\setcounter{dbltopnumber}{9}

\iffalse
\setlength\floatsep{1.25\baselineskip plus 3pt minus 2pt}
\setlength\textfloatsep{1.25\baselineskip plus 3pt minus 2pt}
\setlength\intextsep{1.25\baselineskip plus 3pt minus 2 pt}
\fi

%% bold math in section titles
\makeatletter
\DeclareRobustCommand\bfseries{%
  \not@math@alphabet\bfseries\mathbf
  \fontseries\bfdefault\selectfont\boldmath}
\DeclareRobustCommand*{\bm}[1]{%
    \mathchoice{\bmbox{\displaystyle}{#1}}%
               {\bmbox{\textstyle}{#1}}%
               {\bmbox{\scriptstyle}{#1}}%
               {\bmbox{\scriptscriptstyle}{#1}}}
\DeclareRobustCommand*{\bmbox}[2]{\mbox{\bfseries$#1 #2$}}
\makeatother

\setcapindent{0pt} % to eliminate hanging indent from figure captions

% captions in sans serif
\setkomafont{captionlabel}{\normalfont\sffamily\bfseries}
\setkomafont{caption}{\normalfont\sffamily}
\setkomafont{pagefoot}{\normalfont\sffamily}
\setkomafont{pagenumber}{\normalfont\sffamily}
\setkomafont{pagehead}{\normalfont\sffamily}

%
% longtable caption default
%
\newcommand{\ltbcp}{lngtab}

%
% Modified todo command
%
\newcounter{lzcomm}
\newcommand{\lzcomm}[3][]{%
 % options, initials, comment
 \refstepcounter{lzcomm}%
 { \todo[#1]{%
   \textbf{\uppercase{#2}\thelzcomm:}~#3}}}


%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> LZPaperSupport/packages.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% LZ Paper Support
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% these commands seem to prevent the `too many math alphabets' error
\newcommand\hmmax{0}
\newcommand\bmmax{0}
\usepackage{./LZPaperSupport/hepparticles} % only way I found to unify isotopes
\usepackage[italic]{heppennames}
% order of following seems to work... look out, wrong order can mess things up a lot!
\usepackage{fontspec}
%\setmainfont{STIX2Math}[Extenstion={.otf},Path=./SITX2fonts/,Scale=1]
\setmainfont{STIX2Text}[
Extension={.otf},
Path=./STIX2fonts/,
UprightFont={*-Regular},
BoldFont={*-Bold},
ItalicFont={*-Italic},
BoldItalicFont={*-BoldItalic}]

\usepackage[math-style=ISO]{unicode-math}
\setmathfont{STIX2Math}[Extension={.otf},Path=./STIX2fonts/,Scale=1]
%\usepackage{mathptmx}  % Times fonts - for arxiv submission

%\usepackage{amsmath}

\usepackage[dvipsnames]{xcolor}
\usepackage{colortbl}

\usepackage{siunitx} % manages units... refer to siunitx.cfg for many LZ units


\usepackage{lineno,hyperref}

